Sparse CCA: Adaptive Estimation and Computational Barriers

Canonical correlation analysis is a classical technique for exploring the relationship between two sets of variables. It has important applications in analyzing high dimensional datasets originated from genomics, imaging and other fields. This paper considers adaptive minimax and computationally tractable estimation of leading sparse canonical coefficient vectors in high dimensions. First, we establish separate minimax estimation rates for canonical coefficient vectors of each set of random variables under no structural assumption on marginal covariance matrices. Second, we propose a computationally feasible estimator to attain the optimal rates adaptively under an additional sample size condition. Finally, we show that a sample size condition of this kind is needed for any randomized polynomial-time estimator to be consistent, assuming hardness of certain instances of the Planted Clique detection problem. The result is faithful to the Gaussian models used in the paper. As a byproduct, we obtain the first computational lower bounds for sparse PCA under the Gaussian single spiked covariance model.

==> reduction.tex <==
%!TEX root = appendix-aos.tex




\subsection{A sketch of the reduction scheme}
\label{sec:cb-reduction}




% \subsubsection{Reduction} 
\paragraph{Reduction} 
We now propose our approach to turning an estimator for the sparse CCA problem to a testing procedure for \eqref{eq:pc}.

Let $A\in\{0,1\}^{N\times N}$ be an adjacency matrix sampled either from $H_0^G$ or $H_1^G$. 
Let $n \leq N/12$, and we first construct $n$ pairs of random vectors $(X_i, Y_i)$ where $X_i\in \mathbb{R}^p, Y_i\in \mathbb{R}^m$ with $p=m \geq 2n$. 
The goal here is to ensure that the joint distribution of $\{(X_i,Y_i)\}_{i=1}^n$ is close to $H_0^C$ in \eqref{eq:htCCA} when $A\sim H_0^G$ and to a mixture of the distributions in $H_1^C$ when $A\sim H_1^G$.
This would allow us to turn any test for \eqref{eq:htCCA} to a test for \eqref{eq:pc}, and
the remaining job would be to turn an estimator of the canonical directions to a test for the sparse CCA hypotheses \eqref{eq:htCCA}. To this end,
we construct $n$ auxiliary random vectors $W_i$, which are asymptotically independent of $\{(X_i,Y_i)\}_{i=1}^n$.
When $A\sim H_0^G$, the $W_i$'s are close in distribution to i.i.d.~$N_p(0,I_p)$ vectors.
When $A\sim H_1^G$, the leading eigenvector of the covariance matrix of $W_i$ is essentially identical to the leading canonical directions between the $(X_i, Y_i)$'s.
With the aid of the $W_i$'s, we are able to turn any sparse CCA estimator to a test for the sparse CCA hypothesis \eqref{eq:htCCA}.
% Once we obtain these random vectors, we construct a testing function to detect the planted clique based on a consistent canonical direction estimator.

More precisely, the reduction scheme consists of the following four steps in order. The first three steps generate $\{(X_i,Y_i)\}_{i=1}^n$ and $\{W_i\}_{i=1}^n$ and the last step constructs the test.

% SCCA problem from $A$ with dimension $p=m=N/6$ and sample size $2n=N/6$. To facilitate the construction, let us  prepare some random variables independent from $A$. Generate i.i.d. $\mu_1,...,\mu_{2n}$ distributed by $\bar{h}$. For each $i\in[2n]$, conditioning on $\mu_i$, generate i.i.d. $(B_0)_{i,1},...,(B_0)_{i,2n}$ from $f_{\mu_i,0}$ and i.i.d. $(B_1)_{i,1},...,(B_1)_{i,2n}$ from $f_{\mu_i,1}$. Last but not least, independent from all the randomness above, generate i.i.d. $\wt{Z}_1,...,\wt{Z}_{2n}$ from $N(0,I_p)$. The construction of the SCCA problem consists of two steps.
% 
% \smallskip
% \noindent\textbf{Gaussianization. } Let $A_0\in\{0,1\}^{2n\times 2n}$ be the lower-left part of the matrix $A$. For each $i\in[2n]$ and $j\in[p]$, define
% $$W_{ij}=(B_0)_{ij}\left(1-(A_0)_{ij}\right)+(B_1)_{ij}(A_0)_{ij}.$$
% 
% \smallskip
% \noindent\textbf{Splitting. } Denote the vector $(W_{i1}',...,W_{ip}')'$ by $W_i$. For each $i\in[2n]$, define
% $$X_i=W_i+\wt{Z}_i,\quad Y_i=W_i-\wt{Z}_i.$$



\iffalse
\begin{remark}
To implement the above idea, it is more intuitive to use $\phi_{\mu}$ instead of $\bar{\phi}_{\mu}$ in the definitions of (\ref{eq:f0}) and (\ref{eq:f1}). However, this would make the bounds of Lemma \ref{lem:fixedTV} hold only in a smaller interval of $\mu$ than the one stated in the lemma. The choice of $\bar{\phi}_{\mu}$ allows us to take advantage of the second-order accuracy, and to obtain better approximation in terms of total variation.
\end{remark}
\fi

% Note that the distribution of $(\bar{\epsilon}_1,...,\bar{\epsilon}_{2n})$ is close to that of i.i.d. Bernoulli random variable with mean $k/N$. Therefore, conditioning on $\bar{\gamma}$, when $\bar{\gamma}_j=0$, the density function of $W_{ij}$ is approximately
% \begin{equation}
% \int\left(\frac{1}{2} f_{\mu,0}+\frac{1}{2}f_{\mu,1}\right)\bar{h}(\mu)d\mu\approx N(0,1).\label{eq:eq0}
% \end{equation}
% When $\bar{\gamma}_1=1$, the density function of $W_{ij}$ is approximately
% \begin{equation}
% \int\left(\frac{k}{N}f_{\mu,1}+\left(1-\frac{k}{N}\right)\left(\frac{1}{2} f_{\mu,0}+\frac{1}{2}f_{\mu,1}\right)\right)\bar{h}(\mu)\approx N\left(0,1+\frac{k}{45N(\log N)^2}\right).\label{eq:eq1}
% \end{equation}
% Since the same $\mu_i$ is used for constructing $W_{ij}$ for all $j\in[p]$, the vector $W_i=(W_{i1}',...,W_{ip}')'$ roughly follows $N(0,\xi\theta\theta'+I_p)$ conditioning on $\bar{\gamma}$, for some $\theta\propto \bar{\gamma}$ and some $\xi>0$. Note that this is the Gaussian spiked covariance model used in the SPCA problem. The sparsity is $|\supp(\theta)|=\sum_j\bar{\gamma}_j\asymp k$. 

% Integrating over $\gamma$, the marginal distribution of the $(X_i,Y_i)$'s is close to a mixture of Gaussian single canonical pair model in total variation. 
% In fact, the definitions of the density functions in $f_{\mu,0}$ and $f_{\mu,1}$ can be roughly regarded as solutions to the equations (\ref{eq:eq0}) and (\ref{eq:eq1}).


The materialization of the foregoing discussion leads to the following result
which demonstrates quantitatively that a decent estimator of the leading canonical correlation direction results in a good test (by applying the reduction \eqref{eq:red-1} -- \eqref{eq:red-5}) for the Planted Clique detection problem \eqref{eq:pc}.

\begin{thm}
\label{thm:test-error-cca}
For some sufficiently small constant $c > 0$,
assume $\frac{k^2}{N(\log N)^2}\vee \frac{N(\log N)^5}{k^4}\leq c$, $cN\leq n\leq N/12$ and $p\geq 2n$. 
Then, for any $\wh{u}$ such that
\begin{equation}
\sup_{\mathbb{P}\in \mathcal{P}\left(n,{3k}/{2}, {3k}/{2}, p, p, 1, k\eta_N/8; 4\right)} 
\Prob\left\{L(\wh{u}, u) > \frac{1}{3\times 32^2} \right\} \leq \beta, \label{eq:ce}
\end{equation}
the test $\psi$ defined by \eqref{eq:red-1} -- \eqref{eq:red-5} satisfies
\begin{align*}
\mathbb{P}_{H_0^G}\psi+\mathbb{P}_{H_1^G}(1-\psi) < \beta+\frac{4n}{N}+C(n^{-1}+N^{-1}+e^{-C'k}),
\end{align*}
for sufficiently large $n$
with some constants $C,C'>0$.
\end{thm}

\begin{remark}
% \nb{Both theorems are rigorous. Need some re-wording here. Say one is for continuous data and the other is for discrete data.}
To bridge the gap between \prettyref{thm:test-error-cca} and the desired result in \prettyref{thm:clCCA}, we need to turn the above sketch \eqref{eq:red-1} - \eqref{eq:red-4} into a randomized polynomial-time reduction for discrete data. 
To this end, the major modification is to replace the random number generation in steps 1--3 with their discrete counterparts. For details, see \prettyref{sec:discrete-red} in the supplement.
% \nb{to be rewritten}
% Note that Theorem \ref{thm:test-error-cca} is not for the discretized model, and it does not specify the computational complexity of the reduction scheme.
% The argument in Section \ref{sec:discrete} in the supplementary material. leads to a discretized version of Theorem \ref{thm:test-error-cca}. It says as long as there is a randomized polynomial-time consistent estimator for the canonical direction under the asymptotically equivalent discretized CCA model, then a randomized polynomial-time consistent testing function can be constructed. This can be viewed as a rigorous proof of Theorem \ref{thm:clCCA}.
\end{remark}

\begin{remark}
This section mainly studies computational lower bounds for sparse CCA estimation. Similar results also hold for sparse CCA detection. 
Indeed, if we have a testing procedure for the sparse CCA hypotheses in \eqref{eq:htCCA}, we can replace the fourth reduction step with directly applying the test to the $(X_i,Y_i)$ vectors constructed in \eqref{eq:red-3}.
% One form of sparse CCA detection that we implicitly used in our proposed reduction scheme is (\ref{eq:htCCA}). 
A simple modification of the proof of Theorem \ref{thm:clCCA} then leads to the proof of computational lower bounds for sparse CCA detection.
\end{remark}

\begin{remark}
% Computational lower bounds for sparse PCA based on the Planted Clique hypothesis were established by \cite{berthet2013complexity} and \cite{wang2014statistical}. However, their results are not directly applicable for the well-studied Gaussian spiked covariance model in the literature. The lower bounds were proved for an enlarged space including all distributions possessing a certain rate of tail probability. In contrast, the proposed reduction scheme in this paper is directly targeted for the Gaussian sparse CCA model. 
As we have hinted in (\ref{eq:spca}), a slight variant of the reduction leads to a computational lower bound for sparse PCA under the Gaussian spiked covariance model. This allows us to close the gap in sparse PCA computational lower bounds left by \cite{berthet2013complexity} and \cite{wang2014statistical}. A detailed discussion is given in Section \ref{sec:SPCA} in the supplement. 
\end{remark}

\iffalse
\subsubsection{Theoretical results}

We now materialize the aforementioned intuition by stating rigorous results on the distributions of the $\{(X_i,Y_i)\}_{i=1}^n$ and $\{W_i\}_{i=1}^{n}$ depending on whether $A$ follows $H_0^G$ or $H_1^G$, and by bounding the probabilities of Type I+II errors of the testing procedure in \eqref{eq:red-5} for testing \eqref{eq:pc}.



\fi


\iffalse
\begin{remark}
Theorem \ref{thm:test-error-cca} asserts that as long as there is a consistent estimator of the canonical direction for the Gaussian sparse CCA model, there exists a consistent testing function for the Planted Clique problem. 
 Combining with Hypothesis A, we obtain the computational lower bound of Theorem \ref{thm:clCCA} by letting $n=N/12$, $s_u=s_v=3k/2$ and $\lambda=\frac{k^2}{N(\log N)^2}$.
\end{remark}
\fi










